Unsupervised Discovery of Steerable Factors When Graph Deep Generative Models Are Entangled

Deep generative models (DGMs) have been widely developed for graph data. However, much less investigation has been carried out on understanding the latent space of such pretrained graph DGMs. These understandings possess the potential to provide constructive guidelines for crucial tasks, such as graph controllable generation. Thus in this work, we are interested in studying this problem and propose GraphCG, a method for the unsupervised discovery of steerable factors in the latent space of pretrained graph DGMs. We first examine the representation space of three pretrained graph DGMs with six disentanglement metrics, and we observe that the pretrained representation space is entangled. Motivated by this observation, GraphCG learns the steerable factors via maximizing the mutual information between semantic-rich directions, where the controlled graph moving along the same direction will share the same steerable factors. We quantitatively verify that GraphCG outperforms four competitive baselines on two graph DGMs pretrained on two molecule datasets. Additionally, we qualitatively illustrate seven steerable factors learned by GraphCG on five pretrained DGMs over five graph datasets, including two for molecules and three for point clouds.

==> 10_toy_example_complete.tex <==
\section{Analysis Experiments on Disentanglement} \label{app:sec:toy_example}
In~\Cref{sec:entangled_representation}, we conduct three analysis experiments to conclude that the representation space is not perfectly disentangled in such the setting. In this section, we provide more details and complementary information of these experiments.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment 1: representation visualization} \label{app:sec:toy_example_01}
In~\Cref{sec:entangled_representation}, we force the representation to have dimension of 2, and here we apply PCA on the original pre-trained DGMs, with higher dimensions. As observed from three data types and five DGMs in~\Cref{app:fig:figures_molceules_PCA,app:fig:figures_cloud_points_PCA,app:fig:figures_images_PCA}, we can conclude that, generally, the learnt latnet space is not perfectly disentangled.

% \begin{figure}[H]
% \centering
%     \begin{subfigure}[MoFlow QM9]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/qm9_MolFlow_tsne_369.png}
%     \label{app:fig:MoFlow_QM9_tSNE}}
%     \end{subfigure}
% \hfill
%     \begin{subfigure}[MoFlow ZINC250k]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/zinc250k_MolFlow_tsne_6156.png}
%     \label{app:fig:MOFlow_ZINC250k_tSNE}}
%     \end{subfigure}
% \hfill
%     \begin{subfigure}[HierVAE QM9]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/qm9_HierVAE_tsne_32.png}
%     \label{app:fig:HierVAE_QM9_tSNE}}
%     \end{subfigure}
% \hfill
%     \begin{subfigure}[HierVAE ChEMBL]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/chembl_HierVAE_tsne_32.png}
%     \label{app:fig:HierVAE_ChEMBL_tSNE}}
%     \end{subfigure}
% \caption{
% \todo{tSNE. TBA.}
% }
% \label{app:fig:figures_molecules_tSNE}
% \end{figure}

\begin{figure}[H]
\centering
    \begin{subfigure}[MoFlow QM9]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/qm9_MolFlow_pca_369.png}
    \label{app:fig:MoFlow_QM9_PCA}}
    \end{subfigure}
\hfill
    \begin{subfigure}[MoFlow ZINC250k]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/zinc250k_MolFlow_pca_6156.png}
    \label{app:fig:MOFlow_ZINC250k_PCA}}
    \end{subfigure}
\hfill
    \begin{subfigure}[HierVAE QM9]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/qm9_HierVAE_pca_32.png}
    \label{app:fig:HierVAE_QM9_PCA}}
    \end{subfigure}
\hfill
    \begin{subfigure}[HierVAE ChEMBL]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/chembl_HierVAE_pca_32.png}
    \label{app:fig:HierVAE_ChEMBL_PCA}}
    \end{subfigure}
\vspace{-1.5ex}
\caption{
PCA on the latent space of molecular graph generation models. The two MoFlow models are not perfectly disentangled, while HierVAE shows better independence property. However, this might be caused by the dimension reduction, since in~\Cref{fig:example_01_molecule}, HierVAE is not well disentangled with dimension of two.
}
\label{app:fig:figures_molceules_PCA}
\vspace{-5ex}
\end{figure}

% Below is on the cloud point generative tasks. We sample 2,832 airplanes, 2,458 cars, and 4,612 chairs.
% \begin{figure}[H]
% \centering
%     \begin{subfigure}[PointFlow Airplane]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/airplane_PointFlow_tsne_128.png}
%     \label{app:fig:PointFlow_Airplane_tSNE}}
%     \end{subfigure}
% % \hfill
%     \begin{subfigure}[PointFlow Car]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/car_PointFlow_tsne_128.png}
%     \label{app:fig:PointFlow_Car_tSNE}}
%     \end{subfigure}
% % \hfill
%     \begin{subfigure}[PointFlow Chair]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/chair_PointFlow_tsne_128.png}
%     \label{app:fig:PointFlow_Chair_tSNE}}
%     \end{subfigure}
% \caption{
% \todo{tSNE.}
% }
% \label{app:fig:figures_cloud_points_tSNE}
% \end{figure}

\begin{figure}[H]
\centering
    \begin{subfigure}[PointFlow Airplane]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/airplane_PointFlow_pca_128.png}
    \label{app:fig:PointFlow_Airplane_PCA}}
    \end{subfigure}
% \hfill
    \begin{subfigure}[PointFlow Car]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/car_PointFlow_pca_128.png}
    \label{app:fig:PointFlow_Car_PCA}}
    \end{subfigure}
% \hfill
    \begin{subfigure}[PointFlow Chair]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/chair_PointFlow_pca_128.png}
    \label{app:fig:PointFlow_Chair_PCA}}
    \end{subfigure}
\caption{
PCA on the latent space of point cloud generation models. The latent space of all three datasets are not perfectly disentangled.
}
\label{app:fig:figures_cloud_points_PCA}
\vspace{-5ex}
\end{figure}

% \begin{figure}[H]
% \centering
%     \begin{subfigure}[$\beta$-VAE dSprites]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/dsprite_betaVAE_tsne.png}
%     \label{app:fig:betaVAE_dSprites_tSNE}}
%     \end{subfigure}
%     \begin{subfigure}[StyleGAN FFHQ]
%     {\includegraphics[width=0.23\linewidth]{fig/example_01/ffhq_stylegan2_tsne.png}
%     \label{app:fig:stylegan_ffhq_tSNE}}
%     \end{subfigure}
% \caption{
% \todo{tSNE. TBA.}
% }
% \label{app:fig:figures_images_tSNE}
% \end{figure}

\begin{figure}[H]
\centering
    \begin{subfigure}[$\beta$-VAE dSprites]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/dsprite_betaVAE_pca.png}
    \label{app:fig:betaVAE_dSprites_PCA}}
    \end{subfigure}
    \begin{subfigure}[StyleGAN FFHQ]
    {\includegraphics[width=0.23\linewidth]{fig/example_01/ffhq_stylegan2_pca.png}
    \label{app:fig:stylegan_ffhq_PCA}}
    \end{subfigure}
\caption{
PCA on the latent space of image generation models. The latent space of all both models are not perfectly disentangled.
}
\label{app:fig:figures_images_PCA}
\vspace{-5ex}
\end{figure}
\clearpage







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment 2: disentanglement measure} \label{app:sec:toy_example_02}
\iffalse
\todo{Explain which latent representation space are we plotting w.r.t. the three deep generative models in~\Cref{app:fig:toy_example_02_generative_models}.}
\begin{figure}[H]
\centering
    \begin{subfigure}[VAE]
    {\includegraphics[width=.3\linewidth]{fig/VAE.png}
    \label{app:fig_toy_example_vae}}
    \end{subfigure}
\hfill
    \begin{subfigure}[Flow]
    {\includegraphics[width=.3\linewidth]{fig/Flow.png}
    \label{app:fig_toy_example_flow}}
    \end{subfigure}
\hfill
    \begin{subfigure}[GAN]
    {\includegraphics[width=.3\linewidth]{fig/GAN.png}
    \label{app:fig_toy_example_gan}}
    \end{subfigure}
\caption{VAE in~\Cref{app:fig_toy_example_vae}, Flow-based model in~\Cref{app:fig_toy_example_flow} and GAN in~\Cref{app:fig_toy_example_gan}.
}
\label{app:fig:toy_example_02_generative_models}
\vspace{-3ex}
\end{figure}
\fi


As mentioned in~\Cref{sec:entangled_representation}, we consider the measuring the disentanglement with respect to three types of structured data: molecular graphs, point clouds, and images. Recall that we need to define steerable factors first, so as to measure the disentanglement. Let us introduce them below:
\begin{itemize}[noitemsep,topsep=0pt]
    \item For molecular graphs, we treat the important substructures (a.k.a., motifs or fragments) as factors, and they are extracted using RDKit~\citep{Landrum2016RDKit2016_09_4}. We consider the existence of the following 9 motifs as the binary factor labels: 
    \begin{itemize}[noitemsep,topsep=0pt]
        \item aliphatic hydroxyl groups.
        \item aliphatic hydroxyl groups excluding tert-OH.
        \item aromatic nitrogens.
        \item aromatic amines.
        \item Tertiary amines.
        \item Secondary amines.
        \item amides.
        \item ether oxygens (including phenoxy).
        \item nitriles.
    \end{itemize}
    
    \item For point clouds, we adopt the viewpoint feature histogram (VFH)~\citep{rusu2010fast} implemented in PCL~\citep{Rusu_ICRA2011_PCL}. There are 308 bins in total, where each bin is a histogram of the angles that viewpoint direction makes with each normal. VFH has been widely used as point cloud descriptors, and here we binarize it into factors with:
    \begin{itemize}[noitemsep,topsep=0pt]
        \item We collect the shared non-zero bins from all three datasets (Airplane, Car, and Chair), and ignore the bins where the values distribution are highly skewed. This can give us 75 bins.
        \item Then for each of these selected bins, we use the median value as the threshold to generate the binary factor labels.
    \end{itemize}
    
    \item For images, we consider semantic information (e.g. smiles, glasses) as factors, and they are either pre-defined while generating the synthetic images (dSprites~\citep{dsprites17}) or post-processed by a pre-trained property predictors (FFHQ~\citep{karras2019style}). We consider 6 factors for dSprites: color, shape, scale, orientation, position X, position Y. We consider 40 factors for FFHQ: male, smiling, attractive, wavy hair, young, 5 o\'clock shadow, arched eyebrows, bags under eyes, bald, bangs, big lips, big nose, black hair, blond hair, blurry, brown hair, bushy eyebrows, chubby, double chin, eyeglasses, goatee, gray hair, heavy makeup, high cheekbones, mouth slightly open, mustache, narrow eyes, no beard, oval face, pale skin, pointy nose, receding hairline, rosy cheeks, sideburns, straight hair, wearing earrings, wearing hat, wearing lipstick, wearing necklace, wearing necktie.
\end{itemize}


We follow the~\citep{locatello2019challenging} on considering the following six disentanglement measures:
\begin{itemize}[noitemsep,topsep=0pt]
    \item $\beta$-VAE~\citep{higgins2016beta} evaluates the prediction accuracy of a linear classifier for the index of a fixed factor of variation.
    \item FactorVAE~\citep{kim2018disentangling} addresses the limitations (i.e. corner case) of $\beta$-VAE via introducing a majority voting classifier on a different feature vector. 
    \item MIG~\citep{chen2018isolating} measures the normalized difference between the highest and second highest mutual information between latent dimensions and each steerable factor.
    \item DCI~\citep{eastwood2018framework} disentanglement score measures the average difference from one of the entropy of probability that a latent dimension is useful for predicting a steerable factor (computed by the relative importance score).
    \item Modularity~\citep{ridgeway2018learning} measures whether each latent dimension is dependent on at most one single steerable factor. It computes the average normalized squared difference over the highest and second highest mutual information between each steerable factor and each latent dimension.
    \item SAP~\citep{kumar2018variational} calculates the $R^2$ score of the linear models trained to predict each steerable factor from each latent dimension. 
\end{itemize}

Recall that all six disentanglement measures range from 0 to 1, and higher value means the corresponding space is more disentangled. The results can be found in~\Cref{app:table:disentanglement_measures}. We can conclude that all the values are indeed low on all datasets and models.

\begin{table}[H]
\centering
\small
\caption{
The six mainstream disentanglement metrics on five DGMs and three data types. All measures range from 0 to 1, and higher scores mean more disentangled representation. MoFlow and HierVAE are for molecular graphs, PointFlow is for point clouds, and $\beta$-VAE and StyleGAN are for images.
}
\label{app:table:disentanglement_measures}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l l l c c c c c c}
\toprule
Data Type & Model & Dataset & BetaVAE $\uparrow$ & FactorVAE $\uparrow$ & MIG $\uparrow$ & DCI $\uparrow$ & Modularity $\uparrow$ & SAP $\uparrow$ \\
\midrule
\multirow{4}{*}{Molecular Graphs}
& \multirow{2}{*}{MolFlow} & QM9 & 0.251 & 0.165 & 0.038 & 0.727 & 0.599 & 0.017\\
& & ZINC250k & 0.264 & 0.175 & 0.030 & 0.958 & 0.620 & 0.009 \\
\cmidrule(lr){2-9}
& \multirow{2}{*}{HierVAE} & QM9 & 0.165 & 0.135 & 0.044 & 0.241 & 0.626 & 0.076 \\
& & ChEMBL & 0.159 & 0.130 & 0.023 & 0.113 & 0.604 & 0.026 \\
\midrule
\multirow{3}{*}{Point Clouds} & \multirow{3}{*}{PointFlow} 
& Airplane & 0.022 & 0.025 & 0.029 & 0.160 & 0.745 & 0.022\\
& & Chair & 0.019 & 0.014 & 0.032 & 0.149 & 0.721 & 0.019\\
& & Car & 0.019 & 0.023 & 0.021 & 0.120 & 0.713 & 0.021\\
\midrule
\multirow{3}{*}{Images} &
$\beta$-VAE & dSprites & 0.446 & 0.340 & 0.070 & 0.011 & 0.946 & 0.012\\
\cmidrule(lr){2-9}
& StyleGAN & FFHQ & 0.623 & 0.585 & 0.020 & 0.813 & 0.670 & 0.011\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment 3: visualization of change on latent space} \label{app:sec:toy_example_03}
% To demonstrate the disentanglement level of the learned latent space by deep generative models, we follow the definition of disentanglement and edit the data following the variation of only one single factor in the latent space and observe the changes of edited data. In ~\Cref{app:fig_toy_example3_betavae,app:fig_toy_example3_stylegan,app:fig_toy_example3_moflow_qm9,app:fig_toy_example3_moflow_zinc}, we visualize the results and observe that most of the factors are not disentangled in styleGAN trained on FFHQ and MoFlow trained on QM9. Nevertheless, for $\beta$-VAE trained on dSprites and MoFlow trained on ZINC
If the latent space is perfectly disentangled, then no two latent dimensions will affect the same factors. In other words, if there exist two latent dimensions having the same effect on the same steerable factors, then the corresponding representation space is not perfectly disentangled. Here, we only change one latent dimension and visualize the variance of the reconstructed data caused by this change.
We use $\beta$-VAE trained on dSprites, styleGAN trained on FFHQ, and MoFlow trained on QM9 and ZINC250k as examples.
As shown in~\Cref{app:fig:toy_exmaple_03}, certain changes of different latent dimensions lead to similar variations in the reconstructed data. Therefore, the learned latent space in DGMs is not perfectly disentangled.


\begin{figure}[H]
\centering
    \begin{subfigure}[$\beta$-VAE dSprites]
    {\includegraphics[width=.23\linewidth]{fig/example_03/dSprites_betaVAE_dis.png}
    \label{app:fig_toy_example3_betavae}}
    \end{subfigure}
\hfill
    \begin{subfigure}[styleGAN FFHQ]
    {\includegraphics[width=.23\linewidth]{fig/example_03/stylegan_ffhq1024_stylegan_dis.png}
    \label{app:fig_toy_example3_stylegan}}
    \end{subfigure}
\hfill
    \begin{subfigure}[MoFlow QM9]
    {\includegraphics[width=.23\linewidth]{fig/example_03/qm9_moflow_dis.png}
    \label{app:fig_toy_example3_moflow_qm9}}
    \end{subfigure}
\hfill
    \begin{subfigure}[MoFlow ZINC250k]
    {\includegraphics[width=.23\linewidth]{fig/example_03/zinc250k_moflow_dis.png}
    \label{app:fig_toy_example3_moflow_zinc}}
    \end{subfigure}
\caption{
These four figures demonstrate the variation of edited images and molecules while changing only one latent dimension. All figures illustrate that learnt latent space is not perfectly disentangled.
}
\label{app:fig:toy_exmaple_03}
\end{figure}

==> tables_and_figures/algorithm_train_inference.tex <==

\begin{algorithm}[htb]
\small{
\caption{\small{Training Phase of \model}} \label{alg:model_learning}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Given a pretrained generative model.%, and dataset $\mathcal{X}$.
    \STATE {\bfseries Output:} Learned direction vector $\vd_i$ and function $h(\cdot)$.
    \STATE Select two data points, $\vz^u, \vz^v \in \mathcal{Z}$.
    \FOR{each step size $\alpha$ and each direction $i$}
        \STATE Set $\mz^u_{i, \alpha} = h(\vz^u, \vd_i, \alpha)$.
        \STATE Set $\mz^v_{i, \alpha} = h(\vz^v, \vd_i, \alpha)$.
        \STATE Assign positive to pair $(\mz^u_{i, \alpha}, \mz^v_{i, \alpha})$.
            \FOR{step size $\beta \ne \alpha$ and direction $j \ne i$}
                \STATE Set $\mz^u_{j, \beta} = h(\vz^u, \vd_j, \beta)$.
                \STATE Set $\mz^v_{j, \beta} = h(\vz^v, \vd_j, \beta)$.
                \STATE Assign negative to pair $(\mz^u_{i, \alpha}, \mz^v_{j, \beta})$.
                \STATE Assign negative to pair $(\mz^u_{j, \beta}, \mz^v_{i, \alpha})$.
            \ENDFOR
        \STATE Do SGD w.r.t. \model{} in~\Cref{eq:final_objective}.
    \ENDFOR
\end{algorithmic}
}
\end{algorithm}


\begin{algorithm}[htb]
\small{
\caption{\small{Test Phase of \model}} \label{alg:model_inference}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Given a pre-trained generative model and a selected learned direction vector $\vd$.
    \STATE {\bfseries Output:} A sequence of edited graphs.
    \STATE Sample a molecule with DGM or from a large molecule pool.
    \STATE Encode the molecule to get a latent code $\vz$.\looseness=-1
    \FOR{step size $\alpha \in [-3, 3]$}
        \STATE Do graph edit in the latent space to get $\bar \vz_{i,\alpha} = h(\vz, \vd, \alpha)$.
        \STATE Decode to the graph space with $\bar \vx' = g(\bar \vz_{i,\alpha})$.
    \ENDFOR
    \STATE Output is thus a sequence of edited graphs, $\{\bar \vx'\}$.
\end{algorithmic}
}
\end{algorithm}
